AvalonBench: Evaluating LLMs Playing the Game of Avalon

In this paper, we explore the potential of Large Language Models (LLMs) Agents in playing the strategic social deduction game, Resistance Avalon. Players in Avalon are challenged not only to make informed decisions based on dynamically evolving game phases, but also to engage in discussions where they must deceive, deduce, and negotiate with other players. These characteristics make Avalon a compelling test-bed to study the decision-making and language-processing capabilities of LLM Agents. To facilitate research in this line, we introduce AvalonBench - a comprehensive game environment tailored for evaluating multi-agent LLM Agents. This benchmark incorporates: (1) a game environment for Avalon, (2) rule-based bots as baseline opponents, and (3) ReAct-style LLM agents with tailored prompts for each role. Notably, our evaluations based on AvalonBench highlight a clear capability gap. For instance, models like ChatGPT playing good-role got a win rate of 22.2% against rule-based bots playing evil, while good-role bot achieves 38.2% win rate in the same setting. We envision AvalonBench could be a good test-bed for developing more advanced LLMs (with self-playing) and agent frameworks that can effectively model the layered complexities of such game environments.

==> sections/literature.tex <==
\section{Related Work}

% In this section, we reflect on the prior literature in aligning LLMs towards certain tasks, AI in game-play, interactive LLMs, and human-AI interaction. Our study builds and integrates different parts of these research agendas. 

% Efficient alignment of LLMs is recent major research agenda, since it allows LLMs to complete more specialized tasks and trains them to provide better responses based on limited feedback. A common approach is to use some version of reinforcement learning with human feedback \cite{ouyang2022training}. However, it is costly to create a large human labelled dataset for alignment. One solution to this problem is to have another LLM provide feedback instead of a human \cite{wang2022self}. Instead of having one actor and critic, we can also create a society of actors and have them give each other feedback for alignment \cite{liu2023training}. 





% Making LLMs work together like humans do is also a large inspiration for our work. For example, LLMs can cooperate with one another to complete tasks more effectively \cite{li2023camel}. LLMs have also shown to be able to interact naturally in a simulation society, and plan events such as birthday parties together \cite{park2023generative}. LLMs can also barter with each other, where one LLM tries to sell goods to another, and learn from feedback to barter better \cite{fu2023improving}. 

% Developing AI for game-play has also been a major research agenda, since games provide a easy environment to test intelligence. LLMs by themselves have proven to have some capabilities for cooperation and defection in matrix games \cite{akata2023playing}. We build on the literature of AI in games that require cooperation and communication between more than 2 players, such as diplomacy \cite{gray2020human}. Prior attempts to integrate a reinforcement learning component with a LLM dialogue component have proven to be successful at achieving human level play in diplomacy \cite{meta2022human}. 

% \jon{I think we will need to include more benchmark literature here?}







==> slides.tex <==
% \documentclass[xcolor=dvipsnames]{beamer}
% \usetheme{Madrid}
% \usepackage{amssymb,amsmath, mathrsfs, amsthm, graphicx, hyperref, forest, mathtools}
% \usepackage{booktabs} % for professional tables

% % Uchicago Maroon
% \definecolor{customcolor}{RGB}{136, 0, 0}

% \usecolortheme[named=customcolor]{structure}
% \useoutertheme[subsection=false]{miniframes}

% %\usepackage[margin=1in]{geometry}
% \graphicspath{ {./graphics/} }

% %\usepackage[shortlabels]{enumitem}

% %%graphs
% \usepackage{tikz}
% \usetikzlibrary{arrows,automata}

% \usepackage[latin1]{inputenc}
% \usepackage[ruled,vlined]{algorithm2e}
% %\usepackage[margin=1in]{geometry}
% \usepackage{setspace}
% %\doublespacing

% %Linear Algebra
% \newcommand{\dotmat}[4]{\begin{bmatrix}	#1 & \cdots & #2\\	\vdots & \ddots & \vdots\\	#3&\cdots& #4	\end{bmatrix}}
% \newcommand{\Df}[2][]{D_#1f(#2)}
% \newcommand{\ip}[1]{\langle #1 \rangle}
% \newcommand{\0}{\vec{0}}
% \newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}

% %Analysis Commands
% \newcommand{\R}[1][]{{\mathbb{R}^{#1}}}
% \newcommand{\Q}[1][]{{\mathbb{Q}^{#1}}}
% \newcommand{\N}[1][]{{\mathbb{N}^{#1}}}
% \newcommand{\C}[1][]{{\mathbb{C}^{#1}}}
% \newcommand{\Z}[1][]{{\mathbb{Z}^{#1}}}

% %Permanent Commands
% \newcommand{\lm}[2][t]{\lim\limits_{#1 \rightarrow #2}}
% \newcommand{\lmz}[1][t]{\lim\limits_{#1 \rightarrow 0}}
% \newcommand{\lmi}[1][t]{\lim\limits_{#1 \rightarrow \infty}}
% \newcommand{\zti}{_{0}^{\infty}}
% \newcommand{\vdg}{\vspace{5cm}}
% \newcommand{\ra}{\rightarrow}
% \newcommand{\txt}[1]{&\text{#1}}
% \newcommand{\func}[3]{#1: #2 \rightarrow #3}
% \newcommand{\smm}[1][i]{\sum_{#1 = 0}^{n} }
% \newcommand{\prd}[1][i]{\prod_{#1 = 1}^{n} }

% %Statistics Commands
% \newcommand{\Var}[1]{\mathsf{Var}\big(#1\big)}
% \newcommand{\Cor}[1]{\mathsf{Cor}\big(#1\big)}
% \newcommand{\Cov}[1]{\mathsf {Cov}\big(#1\big)}
% \newcommand{\E}[1]{\mathsf{E}\big[#1\big]}
% \newcommand{\Pb}[1]{\mathsf{P}\big[#1\big]}
% \newcommand{\Bias}[1]{\mathsf{Bias}\big[#1\big]}
% \newcommand{\Dis}[2]{\sim \text{#1}(#2)}

% \newcommand{\Ot}[1]{\mathsf{O}\big[#1\big]}

% %Abstract commands
% %\newcommand{\g}{def}
% \newcommand{\bbm}{\begin{bmatrix}}
% \newcommand{\ebm}{\end{bmatrix}}
% \newcommand{\maximize}[1]{\operatorname{maximize}_{#1} \quad}
% \newcommand{\subjectto}{\text{subject to} \quad}

% %%environments
% %\newenvironment{exercise}[2][Exercise]{\begin{trivlist}
% %\item[\hskip \labelsep {\bfseries #1}\hskip \labelsep {\bfseries #2.}]}{\end{trivlist}}
% %\newenvironment{solution}{\begin{proof}[Solution]}{\end{proof}}
% %\newtheorem*{remark*}{Remark}
% %\theoremstyle{definition}
% %\newtheorem*{definition}{Definition}
% %%\theoremstyle{definition}
% %%\newtheorem{theorem}{Theorem}[section]
% %%\newtheorem{corollary}{Corollary}[theorem]
% %%\newtheorem{lemma}[theorem]{Lemma}
% %%\theoremstyle{definition}
% %%\newtheorem{definition}{Definition}[section]
% %\renewcommand\thesubsection{\thesection\Alph{subsection}}
% %
% %\newenvironment{problem}[2][Problem]{\begin{trivlist}
% %		\item[\hskip \labelsep {\bfseries #1}\hskip \labelsep {\bfseries #2.}]}{\end{trivlist}}
% %
% %\newenvironment{bookproblems}[1][Book Problems]{\begin{trivlist}
% %		\item[\hskip \labelsep {\bfseries #1}{.}]}{\end{trivlist}}


% %\AtBeginSection[]
% %{
% %	\begin{frame}
% %	\frametitle{Table of Contents}
% %	\tableofcontents[currentsection]
% %	\end{frame}
% %}

% \begin{document}

% 	%Below is the information that will be put at the top of the first page of your homework.
% 	\title{From Text to Tactic}
% 	\subtitle{Evaluating LLMs Playing the Game of Avalon}
% 	\author{Jonathan Li}
% 	% \institute{University of Chicago}
% 	\date{\today\\
% %	\vspace{1cm}\tiny \copyright\ 2023 Jonathan Li. Chicago Booth Restricted Materials. All Rights Reserved
% 	} 
	
% 	\frame{\titlepage}
	
% 	\AtBeginSection[]
% 	{
% 		\begin{frame}
% 			\frametitle{Table of Contents}
% 			\tableofcontents[currentsection]
% 		\end{frame}
% 	}
	
% 	\section{Introduction}
	
% 	\begin{frame}
% 		\frametitle{Avalon the Boardgame}
% 		\begin{center}
% 			\includegraphics[scale=0.2]{avalon_components}
% 		\end{center}
% 	\end{frame}

% 	\begin{frame}
% 		\frametitle{Avalon overview}
% 		\begin{center}
% 			\includegraphics[scale=0.4]{graphics/Avalon-06.png}
% 		\end{center}
% 	\end{frame}

% 	\begin{frame}
% 		\frametitle{Required skills to play Avalon}
% 		\begin{center}
% 			\includegraphics[scale=0.4]{graphics/Avalon-07.png}
% 		\end{center}
% 	\end{frame}

%     \begin{frame}{Key Contributions}
%         \begin{itemize}
%             \item We introduce a benchmark \textsc{AvalonBench}~\footnote{The code is available at: \url{https://github.com/jonathanmli/Avalon-LLM}} based on the classic hidden identity game Resistance Avalon to study multi-agent game playing of LLM Agents. % With it, we benchmarked LLMs including GPT-3.5  and Llama2, against deterministic rule-based bots. 
%             \item We demonstrate that current LLM Agents with sophisticated prompt methods do not  possess the deduction, persuasion, negotiation, and deception capabilities yet to play \textsc{Avalon} well. In fact, LLMs could fail against even the simplest of baseline players. 
%             %This highlights the potential for exploring how decision-making techniques can be  integrated with LLMs.
%         \end{itemize}
%     \end{frame}

% 	\section{Model}
	
% 	\begin{frame}
% 		\frametitle{Game flowchart}
% 		\begin{center}
% 			\includegraphics[scale=0.25]{graphics/Avalon_FlowChart_Final.png}
% 		\end{center}
% 	\end{frame}

%     \begin{frame}{Common Human Strategies}
%         Below are some tips that are especially relevant for new players to \textsc{Avalon}. 
        
%         \begin{itemize}
%             \item \textbf{Consistency}
%             \item \textbf{Patience}
%             \item \textbf{Agitation}
%             \item \textbf{Actions speak more than words}
%             \item \textbf{Act ignorant}
%             \item \textbf{Act knowledgeable}
%         \end{itemize}
%     \end{frame}

%     \begin{frame}{Naive Baselines}
% 		\begin{center}
% 			\includegraphics[scale=0.4]{tables/naive_servant.png}
% 		\end{center}
%     \end{frame}

%     \section{Implementation}

%     \begin{frame}{Prompts}
%         \begin{center}
%             \includegraphics[scale=0.4]{tables/prompt_tab.png}
%         \end{center}
%     \end{frame}

%     \begin{frame}{Actions}
%         \begin{align*}
%             \texttt{act\_response } \leftarrow\operatorname{\textsc{LLM}}(\texttt{input}&=\{\texttt{Summary},\texttt{Minutes}\}, \\\texttt{prompt}&=\{\texttt{Rules}, \texttt{Role},\texttt{Request}\})\\
%             \texttt{action} \leftarrow\operatorname{\textsc{LLM}} (\texttt{input}&=\{\texttt{act\_response}\},\\ \texttt{prompt}&=\{\texttt{Parse}\})
%         \end{align*}
%     \end{frame}

%     \begin{frame}{Summary}
%         \begin{align*}
%             \texttt{Summary}_t \leftarrow \textsc{LLM}
%             (\texttt{input   }&= 
%             \{\texttt{Summary}_{t-1}, \texttt{Minutes}_t, \texttt{Outcome}\}, \\ \texttt{prompt}&=\{\texttt{Rules},\texttt{Role},\texttt{Recap}\})
%         \end{align*}
%     \end{frame}

%     \begin{frame}{Discussion}
%         \begin{align*}
%             \texttt{Minutes}_t^{(i)} \leftarrow \textsc{LLM}(\texttt{input}&=\{\texttt{Summary}_t,\texttt{Minutes}_t^{(i-1)}\},\\ \texttt{prompt}&=\{\texttt{Rules},\texttt{Role},\texttt{Discuss}\})
%         \end{align*}
%     \end{frame}
    
%     \section{Experiments}

%     \begin{frame}{Benchmark Results}
%         \begin{center}
%             \includegraphics[scale=0.4]{tables/results.png}
%         \end{center}
%     \end{frame}

%     \begin{frame}{Case Study 1}
%         \begin{center}
%             \includegraphics[scale=0.3]{tables/case_1.png}
%         \end{center}
%     \end{frame}
    
% 	\begin{frame}{Case Study 2}
%         \begin{center}
%             \includegraphics[scale=0.3]{tables/case_2.png}
%         \end{center}
%     \end{frame}

% \end{document}


